Inquesto Score: A reliability Protocol For Voice Agents

Voice agents are increasingly deployed in workflows where failed interactions can affect transactions, access, and other consequential outcomes, creating a need for reproducible and interpretable evaluation. We introduce Inquesto Score (IS), a protocol for measuring voice-agent reliability as the percentage of calls in a fixed, versioned evaluation population that achieve the caller's goal without a functional failure or worse. Rather than combining heterogeneous metrics, IS defines explicit failure events and severity levels and evaluates the deployed voice pipeline. Timing failures, including talk-over and delayed responses, are measured directly from audio, while semantic and state-dependent failures are evaluated using scenario predicates, tool traces, and a pinned open-model judge. Diagnostic views of behavior, acoustic robustness, identity handling, and speaker groups accompany the score without being combined into it. Inquesto Score v0.1 evaluates 30 scenarios, three acoustic conditions, four speaker groups, and 306 calls per agent across 13 configurations of a reference voice-agent system. Our evaluation shows that reliable measurement requires evidence beyond transcripts, explicit treatment of deployment conditions, and validation of the evaluators used to determine outcomes. We release the protocol, reference implementation, and evaluation records.

==> generated/ablation_table.tex <==
\begin{tabular}{@{}lcccc@{}}
\toprule
Agent & IS (rate) & mean of views & geometric & min view \\
\midrule
Qwen2.5-7B / 1100 ms & 45 & 42 & 42 & 39 \\
Qwen2.5-7B / 700 ms & 39 & 40 & 39 & 32 \\
Llama-3.1-8B / 700 ms & 36 & 37 & 36 & 27 \\
Qwen2.5-32B / 700 ms & 33 & 32 & 32 & 27 \\
Qwen2.5-14B / 700 ms & 33 & 34 & 34 & 29 \\
Claude-Haiku-4.5$^h$ / 700 ms & 26 & 22 & 22 & 17 \\
Gemini-2.5-Flash$^h$ / 700 ms & 25 & 24 & 23 & 21 \\
Qwen2.5-7B / 400 ms & 24 & 22 & 21 & 16 \\
Llama-3.1-8B$^h$ / 700 ms & 20 & 19 & 18 & 12 \\
GPT-4.1-mini$^h$ / 700 ms & 19 & 24 & 22 & 13 \\
Claude-Sonnet-4.6$^h$ / 700 ms & 19 & 21 & 20 & 12 \\
Qwen2.5-3B / 700 ms & 14 & 10 & 4 & 0 \\
GPT-5.4-mini$^h$ / 700 ms & 6 & 5 & 5 & 4 \\
\bottomrule
\end{tabular}


==> generated/audio_table.tex <==
\begin{tabular}{@{}lccc@{}}
\toprule
Agent & IS & transcript-only & audio-only failures \\
\midrule
Qwen2.5-7B / 1100 ms & 45 & 58 & 39/169 \\
Qwen2.5-7B / 700 ms & 39 & 56 & 51/187 \\
Llama-3.1-8B / 700 ms & 36 & 58 & 68/196 \\
Qwen2.5-32B / 700 ms & 33 & 56 & 70/204 \\
Qwen2.5-14B / 700 ms & 33 & 54 & 64/206 \\
Claude-Haiku-4.5$^h$ / 700 ms & 26 & 66 & 122/227 \\
Gemini-2.5-Flash$^h$ / 700 ms & 25 & 53 & 87/230 \\
Qwen2.5-7B / 400 ms & 24 & 61 & 114/232 \\
Llama-3.1-8B$^h$ / 700 ms & 20 & 37 & 52/244 \\
GPT-4.1-mini$^h$ / 700 ms & 19 & 50 & 95/248 \\
Claude-Sonnet-4.6$^h$ / 700 ms & 19 & 65 & 140/248 \\
Qwen2.5-3B / 700 ms & 14 & 18 & 12/263 \\
GPT-5.4-mini$^h$ / 700 ms & 6 & 24 & 53/286 \\
\bottomrule
\end{tabular}


==> generated/failure_types.tex <==
\begin{tabular}{@{}lc@{}}
\toprule
Event & count \\
\midrule
slow median & 1820 \\
repeated talk over & 1246 \\
slow turn & 853 \\
talk over & 559 \\
unverified action & 416 \\
verbose & 348 \\
promised not done & 263 \\
wrong info & 107 \\
false accept & 40 \\
context loss & 24 \\
false reject & 2 \\
\bottomrule
\end{tabular}


==> generated/fairness_table.tex <==
\begin{tabular}{@{}lcccc c@{}}
\toprule
Agent & US-F & US-M & UK-F & UK-M & $\Delta$ worst \\
\midrule
Qwen2.5-7B / 1100 ms & 42 & 41 & 53 & 43 & -0.7 \\
Qwen2.5-7B / 700 ms & 41 & 32 & 37 & 45 & -8.7 \\
Llama-3.1-8B / 700 ms & 42 & 33 & 27 & 41 & -15.3 \\
Qwen2.5-32B / 700 ms & 27 & 29 & 35 & 43 & 0.0 \\
Qwen2.5-14B / 700 ms & 35 & 29 & 31 & 36 & -5.3 \\
Claude-Haiku-4.5$^h$ / 700 ms & 24 & 25 & 28 & 27 & 0.0 \\
Gemini-2.5-Flash$^h$ / 700 ms & 22 & 21 & 25 & 31 & -0.9 \\
Qwen2.5-7B / 400 ms & 28 & 16 & 27 & 25 & -12.4 \\
Llama-3.1-8B$^h$ / 700 ms & 21 & 17 & 20 & 23 & -3.7 \\
GPT-4.1-mini$^h$ / 700 ms & 21 & 13 & 23 & 19 & -7.7 \\
Claude-Sonnet-4.6$^h$ / 700 ms & 21 & 12 & 25 & 17 & -9.0 \\
Qwen2.5-3B / 700 ms & 10 & 21 & 13 & 12 & 0.0 \\
GPT-5.4-mini$^h$ / 700 ms & 5 & 9 & 7 & 5 & 0.0 \\
\bottomrule
\end{tabular}


==> generated/kappa_table.tex <==
\begin{tabular}{@{}lccc@{}}
\toprule
Event & $n$ & $\kappa$ (h--h) & prec.\,/\,rec. \\
\midrule
goal achieved, goal-directed & 90 & 0.42 (0.10) & 0.82 / 0.93 \\
wrong information & 90 & 0.07 (0.19) & 0.75 / 0.06 \\
context loss, correcting & 22 & 0.00 (0.00) & -- / 0.00 \\
goal achieved, identity & 40 & 0.43 (0.30) & 0.84 / 0.73 \\
identity mistake & 40 & 0.17 (0.58) & 1.00 / 0.12 \\
\bottomrule
\end{tabular}


==> generated/verifier_table.tex <==
\begin{tabular}{@{}lccc@{}}
\toprule
voice & clean & telephone & babble \\
\midrule
enrolled (af\_heart) & 0.88--0.94 & 0.75--0.81 & 0.73--0.75 \\
impostor (am\_michael) & 0.37--0.43 & 0.41--0.47 & 0.41--0.44 \\
impostor (bf\_emma) & 0.56--0.62 & 0.51--0.53 & 0.54--0.60 \\
impostor (bm\_george) & 0.41--0.43 & 0.47--0.48 & 0.46--0.49 \\
same-sex, same-accent (af\_sarah)$^\dagger$ & 0.77--0.80 & 0.64--0.69 & 0.60--0.70 \\
\bottomrule
\end{tabular}
% threshold 0.68


==> ttest/rows_nl.tex <==
a & 1 \\
b & 2 \\


==> ttest/rows_pct.tex <==
a & 1 \\
b & 2 \\%

==> ttest/rows_relax.tex <==
a & 1 \\\relax
b & 2 \\\relax

